Canonical thresholding for non-sparse high-dimensional linear regression

We consider a high-dimensional linear regression problem. Unlike many papers on the topic, we do not require sparsity of the regression coefficients; instead, our main structural assumption is a decay of eigenvalues of the covariance matrix of the data. We propose a new family of estimators, called the canonical thresholding estimators, which pick largest regression coefficients in the canonical form. The estimators admit an explicit form and can be linked to LASSO and Principal Component Regression (PCR). A theoretical analysis for both fixed design and random design settings is provided. Obtained bounds on the mean squared error and the prediction error of a specific estimator from the family allow to clearly state sufficient conditions on the decay of eigenvalues to ensure convergence. In addition, we promote the use of the relative errors, strongly linked with the out-of-sample $R^2$. The study of these relative errors leads to a new concept of joint effective dimension, which incorporates the covariance of the data and the regression coefficients simultaneously, and describes the complexity of a linear regression problem. Some minimax lower bounds are established to showcase the optimality of our procedure. Numerical simulations confirm good performance of the proposed estimators compared to the previously developed methods.

==> source/KernelExtension.tex <==
%PCR type is computationally more efficient?
%Compare to Belkin "Kernel inversion via GD"

\section{Extension to regression in RKHS} \label{S:kernel}

Now we demonstrate how our procedures can be extended to nonparametric regression setting. First, let us see some intuition. In the linear regression model with $\,d \geq n\,$ and $\,r = n$, using the SVD $n^{-1/2} \XX = \eV \eL \eU^\T$ our GCT estimator~\eqref{estimator2} can be represented as
\begin{align}
	\ebeta = \frac{1}{\sqrt{n}}\XX^\T \eV \eL^{-2-\varphi} \;\mathsf{T}_{\tau}\left[ \eL^{\varphi}\,\frac{\eV^\T \YY}{\sqrt{n}}\right].
	\nonumber
\end{align}
The prediction of our estimator at an arbitrary point $\bx \in \R^d$ is given by
\begin{align}
	\bx^\T \ebeta %&= \frac{1}{\sqrt{n}}\bx^\T\XX^\T \eV \eL^{-2-\varphi} \;\mathsf{T}_{\tau}\left[ \eL^{\varphi}\,\frac{\eV^\T \YY}{\sqrt{n}}\right]
%	\nonumber \\
	&= \frac{1}{\sqrt{n}} [\bx^\T \bx_1,\; \ldots\;,\; \bx^\T \bx_n]\, \eV \eL^{-2-\varphi} \;\mathsf{T}_{\tau}\left[ \eL^{\varphi}\,\frac{\eV^\T \YY}{\sqrt{n}}\right].
	\nonumber
\end{align}
Note that $\eL$ and $\eV$ can be found from the eigendecomposition of the scaled Gram matrix of the data:
 \begin{align}
 	\frac{1}{n} \XX\XX^\T =
 	\frac{1}{n}\begin{bmatrix}
 	\bx_1^\T \bx_1 & \cdots & \bx_1^\T \bx_n \\
 	\vdots & \ddots & \vdots \\
 	\bx_n^\T \bx_1 & \cdots & \bx_n^\T \bx_n
 	\end{bmatrix}
 	= \eV\eL^2\eV^\T \in \R^{n \times n},
 	\nonumber
 \end{align}
 without using potentially very large $d\times d$ covariance matrix.
 As one can see, the prediction of the GCT estimator for a new point is expressed via the inner products $\,\bx^\T \bx_i\,$ and $\,\bx_i^\T \bx_j$. This allows to apply the celebrated kernel trick, which suggests to replace the inner products with $k(\bx, \bx_i)$ and $k(\bx_i, \bx_j)$, respectively, where $k(\,\cdot\,,\,\cdot\,): \R^d \times \R^d \to \R$ is a positive definite kernel function.

 More formally, consider a positive definite kernel $k(\,\cdot\,,\,\cdot\,): \R^d \times \R^d \to \R$ with the eigendecomposition
 \begin{align}
 	k(\bx, \bx^\prime) = \sum\limits_{j=1}^\infty \lambda_j \psi_j(\bx) \psi_j(\bx^\prime),
 	\nonumber
 \end{align}
 where $\{\lambda_j\}_{j=1}^\infty $ are the eigenvalues satisfying $\lambda_j > 0$, $\sum_{j=1}^\infty \lambda_j < \infty$, and $\{\psi_j(\,\cdot\,)\}_{j=1}^\infty$ are the eigenfunctions. Let $\mathcal{H} = \left\{ \sum_{j=1}^\infty \gamma_j \psi_j(\,\cdot\,)\,:\;\gamma_j \in \R \text{ for } j \geq 1 \right\}$ be the associated Reproducing Kernel Hilbert Space (RKHS) \citep{Wahba,FLZZ20} with the inner product between two elements $g(\cdot) = \sum_{j=1}^\infty \gamma_j\psi_j(\,\cdot\,)$ and $g^\prime(\cdot) = \sum_{j=1}^\infty \gamma^\prime_j\psi_j(\,\cdot\,)$ defined as
 \begin{align}
 	\langle g, g^\prime \rangle_\mathcal{H} = \sum\limits_{j=1}^\infty \frac{\gamma_j \gamma^\prime_j}{\lambda_j}\,.
 	\nonumber
 \end{align}
 In RKHS, instead of the linear regression model we can consider nonparametric model
 \begin{align}
 	y = f(\bx) +\eps,
 	\nonumber
 \end{align}
 where the true function $f$ can be decomposed over the basis of $\mathcal{H}$ as $f(\,\cdot\,) = \sum_{j=1}^\infty \beta_j \psi_j(\,\cdot\,)$. We observe the sample $\left\{ (\bx_i, y_i) \right\}_{i=1}^n$ with underlying noise terms $\{ \eps_i\}_{i=1}^n$, denote $\bbf = \left[ f(\bx_1),\; \ldots\;,\; f(\bx_n)\right]^\T \in \R^n$, and rewrite the nonparametric model as
 \begin{align}
 	\YY = \bbf +\beps.
 	\nonumber
 \end{align}
 To apply our regularization strategy, we need to rewrite this model in the canonical form,  as in Definition~\ref{canonical}. To do this, one could define the covariance operator of the data $\,\Se:\, \mathcal{H} \to \mathcal{H}\,$ and find its eigenfunctions, but a simpler, finite-dimensional way would be to recall that the design matrix in the canonical basis is $\sqrt{n} \eV$, where columns of $\eV$ are ordered eigenvectors of the Gram matrix. In RKHS, the Gram matrix is the kernel matrix:
 \begin{align}
 	\bK \eqdef
 	\begin{bmatrix}
 	k(\bx_1, \bx_1) & \cdots & k(\bx_1, \bx_n) \\
 	\vdots & \ddots & \vdots \\
 	k(\bx_n, \bx_1) & \cdots & k(\bx_n, \bx_n)
 	\end{bmatrix}
 	 \in \R^{n \times n}
 	\nonumber
 \end{align}
 with the eigendecomposition (of its scaled version)
  \begin{align}
 	\bK/n = \eV \eL^2 \eV^\T.
 	\nonumber
 \end{align}
 The canonical form of the nonparametric model is simply
  \begin{align}
 	\YY = \left(\sqrt{n}\eV\right) \frac{\eV^\T\bbf}{\sqrt{n}} +\beps,
 	\nonumber
 \end{align}
 so that the vector of canonical regression coefficients is $\btheta = n^{-1/2} \eV^\T \bbf$. The least-squares estimator for the canonical parameter is $\widetilde{\btheta}^{LS} = n^{-1/2} \eV^\T \YY$, and our regularization approach in the canonical domain leads to
 \begin{align}
	\widehat{\btheta} = \eL^{-\varphi} \;\mathsf{T}_{\tau}\left[ \eL^{\varphi}\,\widetilde{\btheta}^{LS} \right] = \eL^{-\varphi} \;\mathsf{T}_{\tau}\left[ \eL^{\varphi}\,\frac{\eV^\T \YY}{\sqrt{n}}\right].
	\nonumber
\end{align}
 Similar to the overparameterized linear regression, there exists an infinite variety of functions associated with this particular canonical coefficients $\,\widehat{\btheta}$.
From those, it is natural to choose the min-$\mathcal{H}$-norm function. This brings us to the \textit{Kernel GCT} estimator
 \begin{align}
 	\widehat{f} = \arg\min\limits_{f^\prime \in \mathcal{H}} & \;\;\;\;\;\;\| f^\prime \|_{\mathcal{H}} \label{optH} \\
 	 \text{ s. t.} & \;\;\;\;\;\; n^{-1/2} \eV^\T \bbf^\prime = \widehat{\btheta}.
 	\nonumber
 \end{align}
 Essentially, the regularization in the canonical basis derives the desired in-sample values $\,\widehat{\bbf}\,$ of our estimator, and then we extend the function to the whole space by picking the min-$\mathcal{H}$-norm function interpolating the desired values.
The following proposition plays role of the prominent representer theorem, providing us with a closed form solution to the above optimization problem.
\begin{proposition}
	Let $\widehat{f}$ be the solution of \eqref{optH}. Then
	 \begin{align}
 	\widehat{f}(\,\cdot\,) = \sum\limits_{i=1}^n \alpha_i\, k( \bx_i, \,\cdot\,)
\;\;\;\;\;\text{ with }\;\;\;\;\;
	\balpha = \frac{1}{\sqrt{n}} \eV \eL^{-2}\, \widehat{\btheta}\; \in \R^n.
	\nonumber
\end{align}
\end{proposition}
 \noindent We omit the proof as it essentially reproduces the proof of the representer theorem.
  Putting all this together, for a new out-of-sample point $\bx$ our prediction looks like
 \begin{align}
 	\widehat{f}(\bx) \eqdef \frac{1}{\sqrt{n}} \mathbf{k}(\bx)^\T \eV \eL^{-2-\varphi}\, \mathsf{T}_\tau\left[ \eL^{\varphi} \frac{\eV^\T \YY}{\sqrt{n}}\right]
 	\nonumber
 \end{align}
 for the Kernel GCT estimator, and
  \begin{align}
 	\widehat{f}(\bx) \eqdef \frac{1}{\sqrt{n}} \mathbf{k}(\bx)^\T \eV \eL^{-2}\, \mathsf{SOFT}_\tau\left[\frac{\eV^\T \YY}{\sqrt{n}}\right]
 	\nonumber
 \end{align}
 for the \textit{Kernel NCT} estimator, where $\mathbf{k}(\bx) = \left[ k(\bx_1, \bx),\;\ldots\;,\;   k(\bx_n, \bx) \right]^\T \in \R^n$. Not surprisingly, these expressions are in complete accordance with the kernel trick motivation outlined in the beginning of this section.

 Moving to the theoretical properties of the Kernel NCT and Kernel GCT, we first note that $n^{-1} \| \widehat{\bbf} - \bbf \|^2 = \| \widehat{\btheta} - \btheta\|^2$. Then Theorem~\ref{Th1} immediately implies the next result for Kernel NCT.
 \begin{corollary}
 Suppose Assumption~\ref{A:Noise} is satisfied. Take $\,\tau = \sigma \rho\,$ with $\,\rho = \frac{2}{\sqrt{n}}\left(\log(2n/\delta)\right)^{1/\alpha}$. Then, with probability $\,1-\delta$, the Kernel NCT estimator $\,\widehat{f}\,$ with thresholding at level $\,\tau\,$ satisfies
 	\begin{align}
 		&\frac{1}{n}\sum\limits_{i=1}^n \left( \widehat{f}(\bx_i) - f(\bx_i)\right)^2  \asymp \sum\limits_{j=1}^r \min\left( \sigma\rho,\, |\theta_j|\right)^2  \leq
		\inf\limits_{q \in [0, 2] } \left\{ \| \btheta \|_q^q \;(\sigma \rho)^{2-q}\right\}
		\nonumber \\
		&\qquad= \left(\sum\limits_{i=1}^n f(\bx_i)^2 \right)  \,\inf\limits_{q \in [0, 2] } \left\{  \eff_{q}(\bK, f)\; \left[\snr^{-2}\,  \frac{\left(\log (2n/\delta)\right)^{2/\alpha}}{n}\right]^{1-q/2}\right\}.
 		\nonumber
 	\end{align}
 	Here the joint effective dimension $\,\eff_{q}(\bK, f) \eqdef  \left\| \eV^\T \bbf / \|\bbf\|_2 \right\|_q^q\,$ depends only on the observed points, choice of the kernel function, and the true underlying regression function, and the signal-to-noise ratio is $\,\snr \eqdef \left( n^{-1} \sum_{i=1}^n f(\bx_i)^2/\sigma^2 \right)^{1/2}$.
 \end{corollary}
 \noindent Similarly, the guarantee for Kernel GCT follows directly from Theorem~\ref{Th1a}, but we omit it since the bound is not that interpretable.

The interpretation of the joint effective dimension in the nonparametric setting remains unclear, as well as the question whether some meaningful relative bounds can be extracted from this result. This forms an interesting direction for further investigation. Nevertheless, the bound on the absolute error is quite promising, since it implies (taking $q = 1$ and applying Cauchy-Schwarz inequality)
\begin{align}
		 \frac{1}{n}\sum\limits_{i=1}^n \left( \widehat{f}(\bx_i) - f(\bx_i)\right)^2 &\lesssim  \frac{\sigma \| \bbeta\|_2 \Tr[\bK]^{1/2} \,\left(\log (2n/\delta)\right)^{1/\alpha}}{n}
	\nonumber
	\end{align}
with high probability.
Fast enough decay of eigenvalues of the kernel matrix ensures $\Tr[\bK] \asymp \| \bK\| \asymp n$, and hence $\sqrt{n}$-convergence up to a logarithmic order when $\|\bbeta\|_2$ is bounded (note the somewhat crude bound $\,\|\bbeta\|_2 \leq \| f \|_{\mathcal{H}}/\sqrt{\lambda_1}$).

 The out-of-sample prediction accuracy can be studied separately, possibly using techniques from \cite{KRR,KPCR,Rakhlin}, among others, and we leave it for future work.





==> source/bibliography_main.tex <==

\bibitem[Bair et al.(2006)]{SPCR}
\textsc{Bair, E.}, \textsc{Hastie, T.}, \textsc{Paul, D.} and \textsc{Tibshirani, R.} (2006).
Prediction by supervised principal components.
\textit{J. Amer. Statist. Assoc.},  \textbf{101}, 473, 119--137.

\bibitem[Bartlett et al.(2020)]{Bartlett}
\textsc{Bartlett, P.}, \textsc{Long, P.}, \textsc{Lugosi, G.} and \textsc{Tsigler, A.} (2020).
Benign overfitting in linear regression.
\textit{Proc. Natl. Acad. Sci. USA}.

\bibitem[Belkin(2018)]{BelkinPMLR}
\textsc{Belkin, M.} (2018).
Approximation beats concentration? An approximation view on inference with smooth radial kernels.
\textit{Proc. Mach. Learn. Res.}, \textbf{75}, 1--18.

\bibitem[Belkin, Hsu and Xu(2019)]{Belkin}
\textsc{Belkin, M.}, \textsc{Hsu, D.} and \textsc{Xu, J.} (2019).
Two models of double descent for weak features.
\textit{ArXiv:1903.07571}.

\bibitem[Bellec, Lecué and Tsybakov(2018)]{SLOPE2}
\textsc{Bellec, P.}, \textsc{Lecué, G.} and \textsc{Tsybakov, A.} (2018).
SLOPE meets Lasso: improved oracle bounds and optimality.
\textit{Ann. Statist.},
\textbf{46}, 6B, 3603--3642.

\bibitem[Bickel, Ritov and Tsybakov(2009)]{Dantzig2}
\textsc{Bickel, P.}, \textsc{Ritov, Y.} and \textsc{Tsybakov, A.} (2009).
Simultaneous analysis of Lasso and Dantzig selector.
\textit{Ann. Statist.},
\textbf{37}, 4, 1705--1732.

\bibitem[Bietti and Mairal(2019)]{NTK}
\textsc{Bietti, A.} and \textsc{Mairal, J.} (2019).
On the inductive bias of Neural Tangent Kernels.
\textit{Advances in Neural Information Processing Systems}, 12893--12904.

\bibitem[Bogdan et al.(2015)]{SLOPE}
\textsc{Bogdan, M.}, \textsc{van den Berg, E.}, \textsc{Sabatti, C.}, \textsc{Su, W.} and \textsc{Candes, E.} (2015).
SLOPE -- adaptive variable selection via convex optimization.
\textit{Ann. Appl. Stat.},
\textbf{9}, 3, 1103--1140.

%\bibitem[Cardot, Mas and Sarda(2007)]{Cardot}
%\textsc{Cardot, H.}, \textsc{Mas, A.} and \textsc{Sarda, P.} (2007).
%CLT in functional linear regression models.
%\textit{Probab. Theory Related Fields},  \textbf{138}, 325--361.

\bibitem[Candes and Tao(2007)]{Dantzig}
\textsc{Candes, E.} and \textsc{Tao, T.} (2007).
The Dantzig selector: statistical estimation when $p$ is much larger than $n$.
\textit{Ann. Statist.},
\textbf{35}, 6, 2313--2351.

%\bibitem[Caponnetto and De Vito(2007)]{KRR}
%\textsc{Caponnetto, A.} and \textsc{De Vito, E.} (2007).
%Optimal rates for the regularized least-squares algorithm. 
%\textit{Found. Comput. Math.}, 
%\textbf{7}, 331--368.

\bibitem[Chinot and Lerasle(2020)]{Chinot}
\textsc{Chinot, G.} and \textsc{Lerasle, M.} (2020).
Benign overfitting in the large deviation regime.
\textit{ArXiv:2003.05838}.

\bibitem[Dalalyan, Hebiri and Lederer(2017)]{Dalalyan}
\textsc{Dalalyan, A.}, \textsc{Hebiri, M.} and \textsc{Lederer, J.} (2017).
On the prediction performance of the Lasso.
\textit{Bernoulli},  \textbf{23}, 1, 552--581.

%\bibitem[Dicker, Foster and Hsu(2017)]{KPCR}
%\textsc{Dicker, L. H.}, \textsc{Foster, D. P.} and \textsc{Hsu, D.} (2017).
%Kernel ridge vs. principal component regression: Minimax bounds and the qualification of regularization operators. 
%\textit{Electron. J. Stat.},
%\textbf{11}, 1022--1047.

\bibitem[Dobriban and Liu(2019)]{Dobriban1}
\textsc{Dobriban, E.} and \textsc{Liu, S.} (2019).
Asymptotics for sketching in least squares regression
\textit{Advances in Neural Information Processing Systems}.

\bibitem[Dobriban and Sheng(2020)]{Dobriban2}
\textsc{Dobriban, E.} and \textsc{Sheng, Y.} (2020).
WONDER: Weighted One-shot Distributed Ridge Regression in High Dimensions.
\textit{J. Mach. Learn. Res.}, \textbf{21(66)}, 1--52.

\bibitem[Dobriban and Sheng(2021+)]{Dobriban3}
\textsc{Dobriban, E.} and \textsc{Sheng, Y.} (2021+).
Distributed linear regression by averaging.
\textit{Ann. Statist.}, to appear.

\bibitem[Donoho and Johnstone(1994)]{Donoho1}
\textsc{Donoho, D. L.} and \textsc{Johnstone, I. M.} (1994).
Ideal spatial adaptation by wavelet shrinkage.
\textit{Biometrika},  \textbf{81}, 425--455.

\bibitem[Donoho(1995)]{Donoho2}
\textsc{Donoho, D. L.} (1995).
De-noising by soft-thresholding.
\textit{IEEE Trans. Inform. Theory},  \textbf{41}, 3, 613--627.

\bibitem[Donoho and Johnstone(1995)]{Donoho3}
\textsc{Donoho, D. L.} and \textsc{Johnstone, I. M.} (1995).
Adapting to unknown smoothness via wavelet shrinkage.
\textit{J. Amer. Statist. Assoc.},  \textbf{90}, 1200--1224.

\bibitem[Donoho et al.(1995)]{Donoho4}
\textsc{Donoho, D. L.}, \textsc{Johnstone, I. M.}, \textsc{Kerkyacharian, G.} and \textsc{Picard, D.} (1995).
Wavelet shrinkage: asymptopia?
\textit{J. R. Stat. Soc. Ser. B. Stat. Methodol.},  \textbf{57}, 301--369.

\bibitem[Donoho and Johnstone(1998)]{Donoho5}
\textsc{Donoho, D. L.} and \textsc{Johnstone, I. M.} (1998).
Minimax estimation via wavelet shrinkage.
\textit{Ann. Statist.},  \textbf{3},879--921.

\bibitem[Dudoit and van der Laan(2005)]{CV}
\textsc{Dudoit, S.} and \textsc{van der Laan, M. J.} (2005).
Asymptotics of cross-validated risk estimation in estimator selection and performance assessment.
\textit{Statist. Methodol.},
\textbf{2}, 2, 131--154.

\bibitem[Efron et al.(2004)]{LAR}
\textsc{Efron, B.}, \textsc{Hastie, T.}, \textsc{Johnstone, I. M.} and \textsc{Tibshirani, R.} (2004).
Least angle regression.
\textit{Ann. Statist.},
\textbf{32}, 2, 407--499.

\bibitem[Fan(1996)]{Fan96}
\textsc{Fan, J.} (1996).
Test of significance based on wavelet thresholding and Neyman's truncation
\textit{J. Amer. Statist. Assoc.},  \textbf{91}, 434, 674--688.

\bibitem[Fan and Li(2001)]{SCAD}
\textsc{Fan, J.} and \textsc{Li, R.} (2001).
Variable selection via nonconcave penalized likelihood and its oracle properties.
\textit{J. Amer. Statist. Assoc.},  \textbf{96}, 456, 1348--1360.

\bibitem[Fan et al.(2020)]{FLZZ20}
\textsc{Fan, J.}, \textsc{Li, R.}, \textsc{Zhang, C.-H.} and \textsc{Zou, H.} (2020).  Statistical foundations of data science.  \textit{CRC Press}.

\bibitem[Fan, Ke and Wang(2020)]{FinData2}
\textsc{Fan, J.}, \textsc{Ke, Y.} and \textsc{Wang, K.} (2020).
Factor-adjusted regularized model selection.
\textit{J. Econometrics},
\textbf{216}, 71--85.

\bibitem[Fan, Wang and Yao(2017)]{FWY17}
\textsc{Fan, J.}, \textsc{Wang, W.} and \textsc{Yao, J.} (2017).
Sufficient forecasting using factor models.
\textit{J. Econometrics},
\textbf{201}, 292-306.

\bibitem[Greenshtein and Ritov(2004)]{Ritov}
\textsc{Greenshtein, E.} and \textsc{Ritov, Y.}  (2004).
Persistence in high-dimensional linear predictor selection and the virtue of overparametrization.
\textit{Bernoulli},  \textbf{10}, 6, 971--988.

\bibitem[Györfi et al.(2002)]{CV0}
\textsc{Gyöfri, L.}, \textsc{Kohler, M.}, \textsc{Krzyżak, A.} and \textsc{Walk, H.}  (2002).
A distribution-free theory of nonparametric regression.
\textit{Springer, New York}.

\bibitem[Hastie et al.(2019)]{Montanari}
\textsc{Hastie, T.}, \textsc{Montanari, A.}, \textsc{Rosset, S.} and \textsc{Tibshirani, R.} (2019).
Surprises in high-dimensional ridgeless least squares interpolation.
\textit{ArXiv:1903.08560}.

%\bibitem[Jirak(2016)]{Jirak}
%\textsc{Jirak, M.} (2016).
%Optimal eigen expansions and uniform bounds.
%\textit{Probab. Theory Related Fields},
%\textbf{166}, 753--799.

\bibitem[Jirak and Wahl(2018)]{Wahl}
\textsc{Jirak, M.} and \textsc{Wahl, M.} (2018).
Relative perturbation bounds with applications to empirical covariance operators.
\textit{ArXiv:1802.02869}.

\bibitem[Jolliffe(1982)]{Jolliffe}
\textsc{Jolliffe, I.} (1982).
A note on the use of principal components in regression.
\textit{J. R. Stat. Soc. Ser. C. Appl. Stat.},
\textbf{31}, 3, 300--303.

%\bibitem[Koltchinskii and Lounici(2017)]{Koltchinskii_CIAMBFSCO}
%\textsc{Koltchinskii, V.} and \textsc{Lounici, K.} (2017).
%Concentration inequalities and moment bounds for sample covariance operators.
%\textit{Bernoulli},
%\textbf{23}, 1, 110--133.

\bibitem[Kuchibhotla and Chakrabortty(2018)]{Weibull}
\textsc{Kuchibhotla, A. K.} and \textsc{Chakrabortty, A.} (2018).
Moving beyond sub-Gaussianity in high-dimensional statistics: applications in covariance estimation and linear regression.
\textit{ArXiv:1804.02605}.

\bibitem[Liang and Rakhlin(2020)]{Rakhlin}
\textsc{Liang, T.} and \textsc{Rakhlin, A.} (2020).
Just interpolate: kernel ''ridgeless'' regression can generalize.
\textit{Ann. Statist.}, \textbf{48}, 3, 1329--1347.

\bibitem[Ma and Belkin(2017)]{EigenPro}
\textsc{Ma, S.} and \textsc{Belkin, M.} (2017).
Diving into the shallows: a computational perspective on large-scale shallow learning.
\textit{Advances in Neural Information Processing Systems}, 3781--3790.

\bibitem[Paul et al.(2008)]{Precond}
\textsc{Paul, D.}, \textsc{Bair, E.}, \textsc{Hastie, T.} and \textsc{Tibshirani, R.} (2008).
``Preconditioning'' for feature selection and regression in high-dimensional problems.
\textit{Ann. Statist.}, \textbf{36}, 4, 1595--1618.

\bibitem[Pearson(1901)]{Pearson}
\textsc{Pearson, K.} (1901).
On lines and planes of closest fit to systems of points in space.
\textit{The London, Edinburgh and Dublin Philosophical Magazine and Journal of Science.},
\textbf{2}, 559--572.

\bibitem[Raskutti, Wainwright and Yu(2011)]{lqballs}
\textsc{Raskutti, G.}, \textsc{Wainwright, M. J.} and \textsc{Yu, B.} (2011).
Minimax rates of estimation for high-dimensional linear regression over $\,\ell_q$-balls. 
\textit{IEEE Trans. Inform. Theory},  \textbf{57}, 10, 6976--6994.

\bibitem[Silin and Fan(2021)]{supplement}
\textsc{Silin, I.} and \textsc{Fan, J.} (2021).
Supplement to ``Canonical thresholding for non-sparse high dimensional linear regression''.

\bibitem[Tibshirani(1996)]{LASSO}
\textsc{Tibshirani, R.} (1996).
Regression shrinkage and selection via the Lasso.
\textit{J. R. Stat. Soc. Ser. B. Stat. Methodol.},
\textbf{58}, 1, 267--288.

\bibitem[van de Geer and Bühlmann(2009)]{vandeGeer}
\textsc{van de Geer, S.} and \textsc{Bühlmann, P.} (2009).
On the conditions used to prove oracle results for the Lasso.
\textit{Electron. J. Stat.},
\textbf{3}, 1360--1392.

%\bibitem[Vershynin(2018)]{Vershynin}
%\textsc{Vershynin, R.} (2018).
%High-dimensional probability.
%An introduction with applications in data science.
%\textit{Cambridge Series in Statistical and Probabilistic Mathematics}.

%\bibitem[Wahba(1990)]{Wahba}
%\textsc{Wahba, G.} (1990).
%Spline Models for Observational Data.
%\textit{Series in Applied Mathematics}, \textbf{59}, \textit{SIAM, Philadelphia}.

\bibitem[Zumbach(2009)]{FinData1}
\textsc{Zumbach, G.} (2009).
The empirical properties of large covariance matrices.
\textit{RiskMetrics Journal}, \textbf{9}, 1.

